Thompson Sampling for Adversarial Bit Prediction

We study the Thompson sampling algorithm in an adversarial setting, specifically, for adversarial bit prediction. We characterize the bit sequences with the smallest and largest expected regret. Among sequences of length $T$ with $k < \frac{T}{2}$ zeros, the sequences of largest regret consist of alternating zeros and ones followed by the remaining ones, and the sequence of smallest regret consists of ones followed by zeros. We also bound the regret of those sequences, the worse case sequences have regret $O(\sqrt{T})$ and the best case sequence have regret $O(1)$. We extend our results to a model where false positive and false negative errors have different weights. We characterize the sequences with largest expected regret in this generalized setting, and derive their regret bounds. We also show that there are sequences with $O(1)$ regret.

==> sections/conclusion.tex <==
This paper studies Thompson sampling in an adversarial bit prediction setting.
We give a full characterization for this particular environment, which enables us to understand the best and worst case behaviour.
Our results show that TS has asymptomatically optimal results in the adversarial bit-prediction setting (i.e. $O(\sqrt{T})$ regret).

We also consider an extension for the bit prediction environment by adding weights to false positive and false negative mistakes. Using the same proof techniques, we managed to characterize this environment as well.

There are several natural directions for further research.
\begin{itemize}
\item In order to get a full understanding of TS in an adversarial environment, we would want to extend the result to an adversarial MAB environment. This is important for a full-information environment as well as a partial one. We expect TS to be asymptotically as good as the known algorithms today.

\item It would be interesting to find lower and upper bounds for the generalized bit-prediction environment. It is also interesting to compare our $O(\sqrt{q(1-q)T})$ regret bound to the performance of other known algorithms in this environment.
\end{itemize}

